Multimodal Language Analysis with Recurrent Multistage Fusion

Computational modeling of human multimodal language is an emerging research area in natural language processing spanning the language, visual and acoustic modalities. Comprehending multimodal language requires modeling not only the interactions within each modality (intra-modal interactions) but more importantly the interactions between modalities (cross-modal interactions). In this paper, we propose the Recurrent Multistage Fusion Network (RMFN) which decomposes the fusion problem into multiple stages, each of them focused on a subset of multimodal signals for specialized, effective fusion. Cross-modal interactions are modeled using this multistage fusion approach which builds upon intermediate representations of previous stages. Temporal and intra-modal interactions are modeled by integrating our proposed fusion approach with a system of recurrent neural networks. The RMFN displays state-of-the-art performance in modeling human multimodal language across three public datasets relating to multimodal sentiment analysis, emotion recognition, and speaker traits recognition. We provide visualizations to show that each stage of fusion focuses on a different subset of multimodal signals, learning increasingly discriminative multimodal representations.

==> figs_tex/attention.tex <==
\begin{figure}[t!]
\centering{
\begin{subfigure}{.45\textwidth}
  	\includegraphics[width=\linewidth, trim={0.5cm 0 0 0},clip]{figs_img/371.png}

\end{subfigure}%
\begin{subfigure}{.45\textwidth}
  	\includegraphics[width=\linewidth, trim={0.5cm 0 0.5cm 0.5cm},clip]{figs_img/373.png}
\end{subfigure}
}
    \caption{ The model learns to suppress and strengthen its attention given different context. (Left fig. )In sample 371, We see a continuous strong focus on a voice modality caused by strong audio input. (Right fig.) In sample 373, none of the vocal or the textual modalities seems to be focused on, but some textual and all the facial modalities are strongly suppressed (the scales are the natural log of the weight).}
    \label{fig:atta}
   % \label{fig:373}
\end{figure}
\begin{figure}[t!]
\centering{
\begin{subfigure}{.45\textwidth}
   	\includegraphics[width=\linewidth, trim={0.5cm 0 0.5cm 0.65cm},clip]{figs_img/467.png}

\end{subfigure}%
\begin{subfigure}{.45\textwidth}
  	\includegraphics[width=\linewidth, trim={0.5cm 0 0.5cm 0.5cm},clip]{figs_img/672.png}
\end{subfigure}
}
    \caption{ The attention reacts to the changes in the input and context in differeent ways. (Left fig. )In sample 476, we observe an abrupt change on the attention starting at time $t_s$, due to the starting of information relevant to sentiment analysis task at that time. (Right fig.) In sample 672, we observe an abrupt change on the attention starting at time $t_s$, due to the starting of information relevant to sentiment analysis task at that time.}
    \label{fig:attb}
   % \label{fig:373}
\end{figure}






==> figs_tex/blocks.tex <==
\begin{figure}[t!]
\centering{
\includegraphics[width=\linewidth]{figs_img/blocks.pdf}}
    \caption{A close-up of the \texttt{HIGHLIGHT} and \texttt{FUSE} operations in the \ourl. $\mathbb{A}$ is the the memory of the \texttt{HIGHLIGHT} module. $\mathbb{S}$ is the memory of the \texttt{FUSE} module. The \texttt{HIGHLIGHT} and \texttt{FUSE} operations are both dependent on representations from previous stages that are stored in $\mathbb{A}$ and $\mathbb{S}$ respectively.}
    \label{fig:blocks}
\end{figure}

==> figs_tex/s1.tex <==
\begin{figure}[t!]
\centering{
\begin{subfigure}{.46\linewidth}
   	\includegraphics[width=\linewidth, trim={1.8cm 1.2cm 3.7cm 0.65cm},clip]{figs_img/49.png}

\end{subfigure}%
\begin{subfigure}{.48\linewidth}
  	\includegraphics[width=\linewidth, trim={3cm 1.2cm 2.0cm 0.5cm},clip]{figs_img/58.png}
\end{subfigure}
}
    \caption{Visualization of the change of the S1 weight across 7 frames on two different videos. In left figure, after the first initialization weighting, we see that the network does not put much weight on any of the modalities across the frames when the sentiment expressed in the video is rather neutral. In the right figure, to the contrary, we observe that the model gives very strong focus on some modalities throughout the video, when the sentiment expressed in the video is more intense.}
    \label{fig:s1}
\end{figure}

==> figs_tex/s2.tex <==
\begin{figure}[t!]
\centering{
\includegraphics[width=\linewidth, trim={0 1.2cm 0 0cm},clip]{figs_img/130.png}}
    \caption{Visualization of the S2 weights across 7 frames and 208 modalities on a sample. While the S1 weights tend to have large variations across time steps, the S2 weights has smaller variation across time steps but have much stronger variations across modalities than the S1 weights. This suggests that what the S2 layer does is to make perturbative corrections to the S1 modalities and thus including higher order non-linear interations in the model.}
    \label{fig:weight_avg}
\end{figure}

==> figs_tex/s3.tex <==
\begin{figure}[t!]
\centering{
\includegraphics[width=\linewidth, trim={0 1.2cm 0 0cm},clip]{figs_img/30.png}}
    \caption{Visualization of the S3 weights across 7 frames and 208 modalities on a sample. We see that the pattern we observed for S2 continues. While the variation across time steps diminishes, the variation across modalities gets large.}
    \label{fig:weight_avg}
\end{figure}

==> figs_tex/single_timestep.tex <==
\begin{figure}[t!]
\centering{
\includegraphics[width=\linewidth, trim={4cm 1.2cm 2.cm 0},clip]{figs_img/time0.png}}
    \caption{Visualization of the total weight changing in $1\times 3$ time steps, 1 denoting actual time step of the frame, and 3 denoting the fusion steps of the recurrent expansion of \pipelines. The y-axis shows the time, and x-axis are the dimensions.}
    \label{fig:single}
\end{figure}

==> figs_tex/vis.tex <==
\begin{figure}[t!]
\centering{
\includegraphics[width=0.8\linewidth]{figs_img/vis.pdf}}
    \caption{Visualization of learned attention weights throughout stages of the multistage fusion process and across time of the multimodal sequence. The learned attention weights are diverse and evolve across stages and time.}
    \label{fig:vis}
\end{figure}

==> figs_tex/weight.tex <==
\begin{figure}[t!]
\centering{
\includegraphics[width=\linewidth, trim={6.5cm 0 0 0},clip]{figs_img/a.png}}
    \caption{Visualization of the total weight changing across $20\times 3$ time steps, 20 denoting actual time step of the data sample, and 3 denoting the time step of the recurrent expansion of our model. The y-axis shows the time, and x-axis are the features.}
    \label{fig:weight}
\end{figure}

==> figs_tex/weight_average.tex <==
\begin{figure}[t!]
\centering{
\includegraphics[width=\linewidth]{figs_img/c.png}}
    \caption{Visualization of the negative log average weight changing across $4 \times 3$ time steps, 4 denoting actual time step of the data sample, and 3 denoting the time step of the recurrent expansion of our model. In the figure, the y-axis shows the time, and x-axis are the features, where row 0 is the average weight of the text feature, 1 is that of the audio feature, and 2 is that of the visual feature.}
    \label{fig:weight_avg}
\end{figure}

==> sections/model.tex <==
\section{\pipelinel}

In this section we describe the \pipelinel \ (\pipelines) for multimodal language analysis (see overview in Figure \ref{fig:model}). Given a set of modalities $\{ l(anguage), v(isual), a(coustic) \}$, the signal from each modality $m \in \{l,v,a\}$ is represented as a temporal sequence $\mathbf{X}^m = \{\textbf{x}_{1}^m, \textbf{x}_{2}^m, \textbf{x}_{3}^m, \cdots, \textbf{x}_{T}^m \}$, where $\textbf{x}^m_{t}$ is the input at time $t$. Each of these temporal sequences $\mathbf{X}^m$ is modeled with a hybrid variant of a recurrent neural network (see Section \ref{sec:LSTHM} for details). At time step $t$, each intra-modal recurrent network will output a unimodal representation $\mathbf{h}^m_t$. The main novelty of our \pipelines \ is in the \ourl \ (\ours) which models cross-modal interactions. The \ours \ uses a recursive approach to fuse all unimodal representations $\mathbf{h}^m_t$ into a multimodal representation $\mathbf{z}_t$. This multimodal representation $\mathbf{z}_t$ is then fed back to each unimodal recurrent network. 

%For each modality $m \in \{l,v,a\}$, a Long Short-term Memory (LSTM) \citep{hochreiter1997long} is utilized to model intra-modal interactions. The input to LSTM $m$ is the sequence $\mathbf{X}^m$ and $\mathbf{h}^m_t$ is the time distributed LSTM output of each modality. The \pipelines \ also contains the \ourl \ (\ours), a neural module that performs multistage fusion to model cross-modal interactions. The \ours \ operates on the representations $\mathbf{h}^m_t$ of each modality and summarizes the learned cross-modal interactions in a cross-modal representation $\mathbf{z}_t$. Figure \ref{fig:model} shows the structure of the \pipelines. 

\subsection{\ourl}

The \ourl \ (\ours) is a modular neural approach that performs multistage fusion to model cross-modal interactions. Multistage fusion is a divide-and-conquer approach which decreases the burden on each stage $k$ of multimodal fusion, allowing each stage of fusion to be performed in a more specialized and effective way. The \ours \ has three main modules: \texttt{HIGHLIGHT}, \texttt{FUSE} and \texttt{SUMMARIZE}. 

The \ours \ has two main modules that are repeated at each stage: \texttt{HIGHLIGHT}, \texttt{FUSE}. The \texttt{HIGHLIGHT} module identifies a subset of multimodal signals from $[\mathbf{h}^l_t,\mathbf{h}^v_t,\mathbf{h}^a_t]$ that will be used for that stage of fusion. The \texttt{FUSE} module then performs 2 tasks: a local fusion of the highlighted features and integration with representations from previous stages.

As an example, in Figure 1, the \texttt{HIGHLIGHT} module selects ``neutral words'' and ``frowning'' expression for the first stage. For stage 2, the \texttt{HIGHLIGHT} module identifies the acoustic feature ``loud voice''. In Figure 1, we show the representations learned after completing both tasks: the local fusion at stage 3 from the highlighted features of ``shrug'' and ``speech elongation'' gives a representation that could be interpreted as ``ambivalence''. The integration with previous stages that deduced the presence of strongly negative emotions then gives a representation closer to ``disappointed''. Both \texttt{HIGHLIGHT} and \texttt{FUSE} modules are realized using memory-based neural networks which enable coherence between stages and grant the program capability to store previously modeled cross-modal interactions. As a final step, a simple module named \texttt{SUMMARIZE} takes the multimodal representation of the final stage and translates it into a cross-modal representation $\mathbf{z}_t$.

%At each stage, dimensions of LSTM outputs $\mathbf{h}^m_t$ are highlighted based on their contribution towards cross-modal interactions. Cross-modal interactions are then fused by building upon previously stored interactions, fully encapsulating the multistage fusion process. We repeat the process in a recurrent manner until all cross-modal interactions are modeled. After all stages are completed, all cross-modal interactions are summarized in a cross-modal representation $\mathbf{z}_t$ that is used to update the LSTM memories.

\subsection{Module Descriptions}

Formally, multistage fusion begins with the concatenation of intra-modal network outputs $\mathbf{h}_t = \bigoplus_{m \in M} \mathbf{h}^m_t$. Our \ours \ approach has memory mechanisms for both the \texttt{HIGHLIGHT} and \texttt{FUSE} modules, \ours \ can be seen as a program with three internal states: $(\mathbb{A},\mathbb{S},\Theta)$. $\mathbb{A}$ is the the memory of the \texttt{HIGHLIGHT} module. $\mathbb{S}$ is the memory of the \texttt{FUSE} module. $\Theta$ denotes the neural network parameters across all modules. After the \texttt{SUMMARIZE} module, the program outputs the cross-modal representation $\mathbf{z}_t$.

\input{figs_tex/blocks.tex}

\texttt{HIGHLIGHT} ($\mathbf{h}_t$): A subset of the multimodal signals represented in $\mathbf{h}_t$ will be automatically highlighted for the local fusion at each stage. Because of the memory present in this module, the highlights at a specific stage will be dependent on previous highlights. Formally, this module is defined as: 
\begin{equation}\label{eq:highlight}
\mathbf{a} = f_{H} (\mathbf{h}_t \ ; \ \mathbb{A},\Theta)
\end{equation}
where $\mathbf{a}$ is a set of attention weights which are inferred based on the previously assigned attention weights $\mathbb{A}$. To fully encapsulate these dependencies, this attention assignment process is performed in a recurrent manner using a Long Short-term Memory (LSTM) \citep{hochreiter1997long} which we call the \texttt{HIGHLIGHT} LSTM. Memory $\mathbb{A}$ of the \texttt{HIGHLIGHT} module is represented by the memory of the \texttt{HIGHLIGHT} LSTM. The recurrence of the \texttt{HIGHLIGHT} LSTM is performed over $K$ stages. The initial memory $\mathbf{c}_{0}^\texttt{HIGHLIGHT}$ is initialized using a network $\mathcal{M}$ that maps $\mathbf{h}_t$ into the LSTM memory space:
\begin{equation}
\mathbf{c}_{0}^\texttt{HIGHLIGHT} = \mathcal{M} (\mathbf{h}_t \ ; \ \Theta)
\end{equation}
This allows the memory mechanism of the \texttt{HIGHLIGHT} LSTM to dynamically adjust to the intra-modal representations $\mathbf{h}_t$. The output of the \texttt{HIGHLIGHT} LSTM $\mathbf{h}_{k}^\texttt{HIGHLIGHT}$ is softmax activated to produce attention weights $\mathbf{a}_{k}$ at every stage $k = 1, \cdots, K$ of the recurrent multistage fusion process:
\begin{equation}
\mathbf{a}_{kj} = \frac{\exp \ (\mathbf{h}_{kj}^\texttt{HIGHLIGHT})}{\sum_{d=1}^{|\mathbf{h}_{k}^\texttt{HIGHLIGHT}|} \exp \ (\mathbf{h}_{kd}^\texttt{HIGHLIGHT})} 
\end{equation}
Highlighting is performed by multiplying the attention weights $\mathbf{a}_{k}$ with the concatenated intra-modal representations:
\begin{equation}\label{eq:discover}
\tilde{\mathbf{h}}_k = \mathbf{h}_t \odot \mathbf{a}_{k}
\end{equation}
where $\tilde{\mathbf{h}}_k$ are the attended multimodal signals that will be used for the local fusion at stage $k$.

\texttt{FUSE} ($\tilde{\mathbf{h}}_k$): The highlighted multimodal signals are fused in a local fusion and integrated with fusion representations from previous stages. Formally, this process is defined as:
\begin{equation}\label{eq:fuse}
\mathbf{s_k} = f_{F} (\tilde{\mathbf{h}}_k \ ; \ \mathbb{S},\Theta)
\end{equation}
We employ a second LSTM, the \texttt{FUSE} LSTM to simultaneously perform local fusion and integration with previous fusion representations. Memory $\mathbb{S}$ of the \texttt{FUSE} module is represented by the \texttt{FUSE} LSTM memory. The \texttt{FUSE} LSTM input gate enables a local fusion while the \texttt{FUSE} LSTM memory and forget gates enable integration with previous fusion results.

\texttt{SUMMARIZE} (): The \ours \ is a recursive process that is performed over multiple stages $k$. After completion, the summarize operation generates a final multimodal representation using all the intermediate representations $\mathbb{S}$ that were stored in the \texttt{FUSE} module. Formally, this process is defined as:
\begin{equation}
\mathbf{z_t} = f_S ( \cdot \ ; \ \mathbb{S},\Theta)
\end{equation}
The memory of \texttt{FUSE} LSTM contains these intermediate representations. At the final stage $K$, a network $\mathcal{S}$ uses $\mathbf{h}^\texttt{FUSE}_K$ to generate the final neural cross-modal representation $\mathbf{z}_t$ at time $t$:
\begin{equation}
\mathbf{z}_t = \mathcal{S}(\mathbf{h}^\texttt{FUSE}_K \ ; \ \Theta)
\end{equation}

Our method has the additional reward of discovering multiple cross-modal interactions via the multiple stages of \texttt{HIGHLIGHT} and \texttt{FUSE}.

\subsection{System of Long Short-term Hybrid Memories}\label{sec:LSTHM}

To synchronize the system of LSTMs using cross-modal representation $\mathbf{z}_{t}$, we employ the system of Long Short-term Hybrid Memories (LSTHMs) \citep{zadeh2018multi}. The LSTHM extends the LSTM formulation to include a multimodal representation $\mathbf{z}_{t}$ in a hybrid memory component:
\begin{align*}
\mathbf{i}_{t+1}^m &= \sigma(\mathbf{W}_i^m\ \mathbf{x}^m_{t+1}+\mathbf{U}^m_i\ \mathbf{h}^m_{t}+\mathbf{V}^m_i\ \mathbf{z}_{t}+\mathbf{b}^m_{i}) \\
\mathbf{f}^m_{t+1} &= \sigma(\mathbf{W}^m_{f}\ \mathbf{x}^m_{t+1} + \mathbf{U}^m_{f}\ \mathbf{h}^m_{t} + \mathbf{V}^m_f\ \mathbf{z}_{t}+\mathbf{b}^m_{f}) \\
\mathbf{o}^m_{t+1} &= \sigma(\mathbf{W}^m_{o}\ \mathbf{x}^m_{t+1} + \mathbf{U}^m_{o}\ \mathbf{h}^m_{t} + \mathbf{V}^m_o\ \mathbf{z}_{t}+\mathbf{b}^m_{o}) \\
\bar{\mathbf{c}}_{t+1}^m &= \mathbf{W}_{\bar{c}}^m\ \mathbf{x}^m_{t+1} + \mathbf{U}_{\bar{c}}^m\ \mathbf{h}^m_{t} + \mathbf{V}_{\bar{c}}^m\ \mathbf{z}_{t} + \mathbf{b}^m_{\bar{c}} \\
\mathbf{c}^m_{t+1} &= \mathbf{f}^m_t \odot \mathbf{\mathbf{c}}^m_{t} + \mathbf{i}^m_t \odot tanh(\bar{\mathbf{c}}_{t+1}^m) \\
\mathbf{h}^m_{t+1} &= \mathbf{o}^m_{t+1} \odot tanh(\mathbf{c}^m_{t+1})
\end{align*}
where $\sigma$ is the (hard-)sigmoid activation function, $tanh$ is the tangent hyperbolic activation function, $\odot$ denotes element-wise multiplication. $\mathbf{i},\mathbf{f}$ and $\mathbf{o}$ are the input, forget and output gates respectively. $\bar{\mathbf{c}}_{t+1}^m$ is the proposed update to the hybrid memory $\mathbf{c}^m_t$ at time $t+1$ and $\mathbf{h}^m_t$ is the time distributed output of each modality. $\mathbf{z}_t$ is the cross-modal representation modeled by the \ourl. The hybrid memory $\mathbf{c}^m_t$ contains both intra-modal interactions in individual modalities $\mathbf{x}^m_t$ as well as cross-modal interactions from the cross-modal representation $\mathbf{z}_t$.

\subsection{Optimization}
In our experiments, the final representations $\mathcal{E}$ from multimodal temporal sequences are (1) the last outputs from the LSTHMs $\{ \mathbf{h}^m_T : m \in M \}$ and (2) the last cross-modal representation $\mathbf{z}_T$. These summarize the modeled intra-modal and cross-modal representations from times $1, \cdots , T$:
\begin{equation}
\mathcal{E} = (\bigoplus_{m \in M} \mathbf{h}^m_T) \bigoplus \mathbf{z}_T
\end{equation}
where $\bigoplus$ denotes vector concatenation. $\mathcal{E}$ can then be used as a multimodal representation for supervised or unsupervised analysis of human multimodal language. \pipelines \ is differentiable end-to-end which allows the model to be learned efficiently using gradient descent approaches. We apply dropout training \citep{Srivastava:2014:DSW:2627435.2670313} for dense layers but not for recurrent layers \citep{Zaremba}. We train our model with the Adam optimizer \citep{kingma2014adam} and apply soft targets for classification tasks \citep{Hinton2015,PereyraTCKH17}. The code is publicly available at \url{<anonymous>}. 



==> sections/related_works.tex <==
\section{Related Work}
\label{Related Work}
Previous approaches in human multimodal language modeling can be categorized as follows:

\noindent \textbf{Early Fusion}: In early fusion methods, multimodal input feature concatenation is used to simplify intra-modal and cross-modal interaction discovery. These approaches adapt classical supervised learning methods to discover both intra-modal and cross-modal interactions without specific model design~\cite{wang2016select,poria2016convolutional}. Some early fusion approaches remove the time factor as well~\cite{zadeh2016multimodal,morency2011towards}. These methods tend to overfit on input data~\cite{xu2013survey} without discovering generalizable intra-modal and cross-modal interactions.

\noindent \noindent \textbf{Late Fusion}: Late fusion methods learn separate models for each modality and combine the outputs using decision voting~\cite{torstenptsd,Nojavanasghari:2016:DMF:2993148.2993176}. While these methods are generally strong in discovering intra-modal interactions, simple decision voting is unable to discover the complex combinations that are present in cross-modal interactions.

\noindent \textbf{Non-temporal Models}: These models simplify the problem by summarizing temporal observations with simpler statistics~\citep{contextmultimodalacl2017,perez2013utterance,wollmer2013youtube}. Often each modality is represented by averaging temporal information through time~\citep{abburi2016multimodal,Nojavanasghari:2016:DMF:2993148.2993176}. These approaches often have trouble modeling long sequences since the averages statistics do not properly model the temporal intra-modal and cross-modal dynamics.

\input{figs_tex/model.tex}

%Computational analysis of human multimodal language is a recent trend in NLP. Studies have suggested using information from language, vision and acoustic modalities can improve the performance of NLP models. Sentiment analysis has been extensively studied in a multimodal framework \cite{tensoremnlp17,poriaa2017multi,perez2013utterance,morency2011towards}. Recently other studies have reported successfully using multimodal language data for tasks such such as emotion recognition \cite{porianaacl2018,yu2017temporally} as well as personality traits recognition \cite{park2014computational}. Overarching studies have addressed an array of NLP tasks using multimodal language data and novel machine learning techniques including Memory Fusion Networks \cite{zadeh2018memory} and Multi-attention Recurrent Network (MARN) \cite{zadeh2018multi} for multimodal tasks. 

\noindent \textbf{Multimodal Temporal Learning}: Extensions of Hidden Markov Models \cite{baum1966statistical}, Conditional Random Fields~\citep{Lafferty:2001:CRF:645530.655813}, and Hidden Conditional Random Fields \cite{Quattoni:2007:HCR:1313053.1313265,morency2007latent} have been proposed for multimodal temporal learning \cite{song2012multi,song2013action}. Long Short-term Memories (LSTMs) have also been extended for multimodal settings \cite{rajagopalan2016extending} and by learning binary gating mechanisms to remove noisy modalities \cite{Chen:2017:MSA:3136755.3136801}. Recently, more advanced models were proposed to model intra-modal and cross-modal interactions. These were performed using external multimodal memory mechanisms \cite{zadeh2018memory} or multiple attention coefficient assignments for multiple cross-modal interactions \cite{zadeh2018multi}. While these models attempted to model intra-modal and cross-modal interactions, none modeled cross-modal interactions across multiple stages. They make the assumption that individual cross-modal interactions should be discovered all at once rather than across multiple stages, an assumption we show to be less suitable through our empirical evaluations.




==> sections/results.tex <==
\section{Results and Discussion}

%\input{tables/pom_small.tex}

Results on CMU-MOSI, IEMOCAP and POM are presented in Tables~\ref{mosi},~\ref{iemocap} and~\ref{pom} respectively\footnote{results for all baseline models are in supplementary.}. We achieve state-of-the-art or competitive results for all domains, highlighting \pipelines's capability in human multimodal language analysis. We observe that \pipelines \ does not improve results on IEMOCAP neutral emotion and the approach outperforming RMFN is a memory-based fusion baseline~\citep{zadeh2018memory}. We believe that this is because neutral expressions are quite idiosyncratic. Some people may always look angry given their facial configuration (e.g., natural eyebrow raises of actor Jack Nicholson). In these situations, it becomes useful to compare the current image with a memorized or aggregated representation of the speaker's face. Therefore, it can help create an internal model of how the person is looking when neutral and memory-based fusion methods are beneficial.

%\textbf{Multimodal Sentiment Analysis:} We summarize results on the CMU-MOSI dataset in Table \ref{mosi}. We achieve state-of-the-art results for this dataset in all metrics using the \pipelines. This highlights our model's capability in understanding sentiment from multimodal language.

%\textbf{Multimodal Emotion Recognition:} Our results on the IEMOCAP dataset are presented in Table \ref{iemocap}. \pipelines \ achieves state-of-the-art performance in speaker emotion recognition over the emotions of happy, sad, angry and neutral.

%\textbf{Multimodal Speaker Traits Recognition:} Table \ref{pom} shows the performance of the \pipelines \ on POM dataset, where it achieves state-of-the-art accuracies on recognizing multiple speaker traits including confidence, persuasiveness and credibility. 



==> tables/mmmo+you+moud.tex <==
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
\definecolor{gg}{RGB}{45,190,45}

\begin{table}[tb]
\fontsize{7.5}{10}\selectfont
%\centering
\setlength\tabcolsep{1.3pt}
\begin{tabular}{l : *{2}{K{0.93cm}} : *{2}{K{0.93cm}} : *{2}{K{0.93cm}}}
\Xhline{3\arrayrulewidth}
Dataset & \multicolumn{2}{c:}{\textbf{ICT-MMMO}} & \multicolumn{2}{c:}{\textbf{YouTube}} & \multicolumn{2}{c}{\textbf{MOUD}} \\
%\cmidrule(lr{.5em}){2-3}  \cmidrule(lr{.5em}){4-5} \cmidrule(lr{.5em}){6-7} 
Task & \multicolumn{2}{c:}{Sentiment} & \multicolumn{2}{c:}{Sentiment} & \multicolumn{2}{c}{Sentiment} \\
Method        	& A$^{2}$ & F1 & A$^{3}$ & F1 & A$^{2}$ & F1 \\ 
\Xhline{0.5\arrayrulewidth}
%Random			& 33.90 & 31.44 & 45.28 & 45.87\\
Majority		& 40.0 & 22.9 & 42.4 & 25.2 & 60.4 & 45.5\\
RF				& 70.0 & 69.8 & 33.3 & 32.3 & 64.2 & 63.3\\
SVM     		& 68.8 & 68.7 & 42.4 & 37.9 & 59.4 & 45.5\\
THMM			& 53.8	& 53.0 & 42.4 & 27.9 & 61.3 & 57.0\\
%MVCCA-C			&  &  && \\
%C-MKL			& 80.0 & 72.4 & 50.2 & 50.8 & 74.0 & 74.7 \\
% EF-HCRF$_{(\star)}$	& 73.8$_{\textrm{(l)}}$ & 73.1$_{\textrm{(l)}}$ & 45.8$_{\textrm{(l)}}$ & 45.0$_{\textrm{(l)}}$ & 54.7$_{\textrm{(h)}}$ & 54.7$_{\textrm{(h)}}$ \\
% MV-HCRF$_{(\star)}$	& 68.8$_{\textrm{(l)}}$ & 67.1$_{\textrm{(l)}}$ & 44.1$_{\textrm{(s)}}$ & 44.0$_{\textrm{(s)}}$	& 60.4$_{\textrm{(l)}}$ & 47.8$_{\textrm{(l)}}$ \\
EF-HCRF			& 50.0 & 50.3 & 44.1 & 43.8 & 54.7 & 54.7 \\
EF-LDHCRF		& 73.8 & 73.1 & 45.8 & 45.0 & 52.8 & 49.3 \\
MV-HCRF			& 36.3 & 19.3 & 27.1 & 19.7 & 60.4 & 45.5 \\
MV-LDHCRF		& 68.8 & 67.1 & 44.1 & 44.0	& 53.8 & 46.9 \\
CMV-HCRF		& 36.3 & 19.3 & 30.5 & 14.3 & 60.4 & 45.5 \\
CMV-LDHCRF		& 51.3 & 51.4 & 42.4 & 42.0 & 53.8 & 47.8 \\
EF-HSSHCRF		& 50.0 & 51.3 & 37.3 & 35.6 & 52.8 & 49.3 \\
MV-HSSHCRF		& 62.5 & 63.1 & 44.1 & 44.0 & 47.2 & 46.4 \\
DF   			& 65.0 & 58.7 & 45.8 & 32.0 & 67.0 & 67.1 \\
%EF-LSTM$_{(\star)}$	& 72.5$_{\textrm{(s)}}$ & 70.9$_{\textrm{(s)}}$ & 44.1$_{\textrm{(-)}}$ & 43.6$_{\textrm{(-)}}$ & 67.0$_{\textrm{(-)}}$ & 64.3$_{\textrm{(-)}}$ \\
EF-LSTM   		& 66.3 & 65.0 & 44.1 & 43.6 & 67.0 & 64.3 \\
EF-SLSTM		& 72.5 & 70.9 & 40.7 & 41.2	& 56.6 & 51.4 \\
EF-BLSTM 		& 63.8 & 49.6 & 42.4 & 38.1 & 58.5 & 58.9 \\
EF-SBLSTM 		& 62.5 & 49.0 & 37.3 & 33.2 & 63.2 & 63.3 \\
MV-LSTM			& 72.5 & 72.3 & 45.8 & 43.3 & 57.6 & 48.2 \\
BC-LSTM    		& 70.0 & 70.1 & 45.0 & 45.1 & 72.6 & 72.9 \\ 
TFN      		& 72.5 & 72.6 & 45.0 & 41.0 & 63.2 & 61.7 \\ 
MARN			& 71.3 & 70.2 & 48.3 & 44.9 & 81.1 & 81.2 \\ 
MFN				& 70.0 & 69.3 & 51.7 & 51.6 & 81.1 & 80.4 \\
DFG      		& {76.3} & {76.2} & {55.0} & {53.5} & {81.1} & {80.9} \\ 
\Xhline{0.5\arrayrulewidth}
{\ours}      	& \textbf{68.8}	& \textbf{67.1}& \textbf{50.0}& \textbf{46.2}& \textbf{78.3}& \textbf{78.5}\\ 
\Xhline{0.5\arrayrulewidth}
$\Delta_{SOTA}$	& \textcolor{gg}{$\uparrow $ \textbf{2.5}} & \textcolor{gg}{$\uparrow $ \textbf{3.1}} & \textcolor{gg}{$\uparrow $ \textbf{9.2}} & \textcolor{gg}{$\uparrow $ \textbf{8.4}} & \textcolor{gg}{$\uparrow $ \textbf{8.5}} & \textcolor{gg}{$\uparrow $ \textbf{8.0}} \\ 
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Sentiment prediction results on ICT-MMMO, YouTube and MOUD test sets. The best results are highlighted in bold and $\Delta_{SOTA}$ shows the change in performance over previous state of the art. Improvements are highlighted in green. The \ours \ significantly outperforms the current state of the art across all evaluation metrics.}
\label{mmmo+you+moud}
\end{table}

==> tables/pom.tex <==
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
\definecolor{gg}{RGB}{45,190,45}

\begin{table*}[!htbp]
\fontsize{7}{10}\selectfont
%\centering
\setlength\tabcolsep{1.3pt}
\begin{tabular}{l : *{16}{K{0.82cm}}}
\Xhline{0.5\arrayrulewidth}
Dataset & \multicolumn{16}{c}{\textbf{POM Speaker Personality Traits}} \\
Task & \multicolumn{1}{c}{Con} & \multicolumn{1}{c}{Pas} & \multicolumn{1}{c}{Voi} & \multicolumn{1}{c}{Dom} & \multicolumn{1}{c}{Cre} & \multicolumn{1}{c}{Viv} & \multicolumn{1}{c}{Exp} & \multicolumn{1}{c}{Ent} & \multicolumn{1}{c}{Res} & \multicolumn{1}{c}{Tru} & \multicolumn{1}{c}{Rel} & \multicolumn{1}{c}{Out} & \multicolumn{1}{c}{Tho} & \multicolumn{1}{c}{Ner} & \multicolumn{1}{c}{Per} & \multicolumn{1}{c}{Hum}\\
Metric & A$^7$ & A$^7$ & A$^7$ & A$^7$ & A$^7$ &  A$^7$ & A$^7$ & A$^7$ & A$^5$ & A$^5$ & A$^5$ & A$^5$ & A$^5$ & A$^5$ & A$^7$ & A$^5$  \\ 
\Xhline{0.5\arrayrulewidth}
Majority		& 19.2&20.2&30.5&18.2&21.7&25.6&26.1&19.7&29.6&44.3&39.4&36.0&31.0&24.1&20.7&6.9 \\
SVM     		&  20.6 & 20.7 & 32.0 & 35.0 & 25.1 & 29.1 & 26.6 & 31.5 & 34.0 & 50.2 & 49.8 & 42.9 & 39.9 & 41.4 & 28.1 & 36.0 \\
RF     			&  26.6&27.1&29.6&26.1&23.2&23.6&26.6&26.1&34.0&53.2&40.9&32.5&37.4&36.0&25.6&40.4  \\
THMM    		& 24.1&15.3&19.2&29.1&27.6&26.1&18.7&12.3&22.7&31.0&31.5&30.0&30.0&27.1&17.2&24.6 \\
DF   & 25.6&24.1&33.0&34.0&26.1&32.0&26.6&29.6&30.0&53.7&50.2&39.4&37.9&42.4&26.6&34.5\\
%EF-LSTM$_{(\star)}$	& 25.1$_{\textrm{(b)}}$&30.5$_{\textrm{(sb)}}$& 34.0$_{\textrm{(b)}}$ & 36.9$_{\textrm{(s)}}$&29.6$_{\textrm{(b)}}$&32.5$_{\textrm{(sb)}}$&31.0$_{\textrm{(sb)}}$&33.5$_{\textrm{(b)}}$&33.5$_{\textrm{(sb)}}$&52.7$_{\textrm{(sb)}}$&48.3$_{\textrm{(-)}}$&40.4$_{\textrm{(s)}}$&42.4$_{\textrm{(-)}}$&44.8$_{\textrm{(sb)}}$&25.6$_{\textrm{(sb)}}$&39.4$_{\textrm{(b)}}$ \\
EF-LSTM   & 20.7&27.6&31.5&35.0&25.1&31.0&25.1&29.1&30.0&48.3&48.3&38.4&42.4&40.4&25.6&36.0\\
EF-SLSTM	& 22.2&28.6&30.5&36.9&27.1&32.0&27.6&27.6&32.5&49.3&46.8&40.4&39.9&41.9&22.7&35.0 \\
EF-BLSTM & 25.1&26.1&34.0&32.0&29.6&31.0&25.6&33.5&30.0&52.2&46.3&34.0&41.9&42.9&25.6&39.4\\
EF-SBLSTM & 23.2&30.5&29.1&31.0&27.6&32.5&31.0&25.1&33.5&52.7&47.8&38.4&39.4&44.8&25.6&38.9\\
MV-LSTM 		& 25.6&28.6&28.1&34.5&25.6&32.5&29.6&29.1&33.0&52.2&50.7&38.4&37.9&42.4&26.1&38.9\\
BC-LSTM    		& 26.6&26.6&31.0&33.0&27.6&36.5&30.5&29.6&33.0&52.2&47.3&37.9&45.8&36.0&27.1&36.5\\ 
TFN      		& 24.1&31.0&31.5&34.5&24.6&25.6&27.6&29.1&30.5&38.9&35.5&37.4&33.0&42.4&27.6&33.0\\ 
MARN		& 29.1&33.0&-&38.4&31.5&-&-&33.5&36.9&55.7&52.2&-&-&47.3&31.0&44.8 \\
MFN			& {34.5}&{35.5}&{37.4}&\textbf{41.9}&{34.5}&{36.9}&{36.0}&\textbf{37.9}&{38.4}&\textbf{57.1}&{53.2}&\textbf{46.8}&{47.3}&{47.8}&{34.0}&\textbf{47.3} \\
%DFG			& {35.5}&{35.0}&{36.5}&{41.9}&{32.0}&{36.9}&{37.4}&{36.9}&{37.4}&{55.2}&{53.7}&{45.8}&{48.3}&{46.3}&{34.5}&{43.8} \\
\Xhline{0.5\arrayrulewidth}
{\pipelines }  &  \textbf{37.4} & \textbf{38.4} &\textbf{37.4} &{39.4} &\textbf{37.4} &\textbf{38.9} &\textbf{38.9} &{36.9} &\textbf{39.4} &{56.7} &\textbf{53.7} &{46.3} &\textbf{48.3} &\textbf{48.3} &\textbf{35.0} &{46.8}\\
\Xhline{0.5\arrayrulewidth}
$\Delta_{SOTA}$	& \textcolor{gg}{$\uparrow $ \textbf{2.9}} & \textcolor{gg}{$\uparrow $ \textbf{2.9}} & \textcolor{gg}{$\uparrow $ \textbf{0.0}} & \textcolor{gray}{$\downarrow $ \textbf{2.5}} & \textcolor{gg}{$\uparrow $ \textbf{2.9}} & \textcolor{gg}{$\uparrow $ \textbf{2.0}} & \textcolor{gg}{$\uparrow $ \textbf{2.9}} & \textcolor{gray}{$\downarrow $ \textbf{1.0}} & \textcolor{gg}{$\uparrow $ \textbf{1.0}} & \textcolor{gray}{$\downarrow $ \textbf{0.4}} & \textcolor{gg}{$\uparrow $ \textbf{0.5}} & \textcolor{gray}{$\downarrow $ \textbf{0.5}} & \textcolor{gg}{$\uparrow $ \textbf{1.0}} & \textcolor{gg}{$\uparrow $ \textbf{0.5}} & \textcolor{gg}{$\uparrow $ \textbf{1.0}} & \textcolor{gray}{$\uparrow $ \textbf{0.5}} \\ 
\Xhline{0.5\arrayrulewidth}
%& 32.5&37.4&36.9&40.9&33.0&36.5&33.5&36.5&38.9&55.7&52.7&43.8&47.8&47.3&25.6&33.5&45.8\\   \hline
\end{tabular}
\end{table*}

\begin{table*}[!htbp]
\fontsize{7}{10}\selectfont
%\centering
\setlength\tabcolsep{1.3pt}
\begin{tabular}{l : *{16}{K{0.82cm}}}
\Xhline{0.5\arrayrulewidth}
Dataset & \multicolumn{16}{c}{\textbf{POM Speaker Personality Traits}} \\
Task & \multicolumn{1}{c}{Con} & \multicolumn{1}{c}{Pas} & \multicolumn{1}{c}{Voi} & \multicolumn{1}{c}{Dom} & \multicolumn{1}{c}{Cre} & \multicolumn{1}{c}{Viv} & \multicolumn{1}{c}{Exp} & \multicolumn{1}{c}{Ent} & \multicolumn{1}{c}{Res} & \multicolumn{1}{c}{Tru} & \multicolumn{1}{c}{Rel} & \multicolumn{1}{c}{Out} & \multicolumn{1}{c}{Tho} & \multicolumn{1}{c}{Ner} & \multicolumn{1}{c}{Per} & \multicolumn{1}{c}{Hum}\\
Metric & \multicolumn{16}{c}{MAE} \\ 
\Xhline{0.5\arrayrulewidth}
Majority & 1.483&1.268&1.089&1.167&1.260&1.158&1.164&1.231&1.166&0.743&0.753&0.872&0.939&1.181&1.328&1.774 \\
SVM	& 1.071&1.159&0.938&0.865&1.036&1.043&1.031&0.988&0.877&0.536&0.594&0.702&0.728&0.714&1.110&0.801\\
DF		& 1.033&1.083&0.899&0.870&1.039&0.997&1.027&0.967&0.884&0.534&0.591&0.698&0.732&0.695&1.086&0.768 \\
EF-LSTM			&  1.035&1.067&0.911&0.889&1.022&0.981&0.990&0.976&0.880&0.556&0.594&0.700&0.712&0.706&1.084&0.768\\
EF-SLSTM & 1.047&1.069&0.924&0.880&1.040&0.990&1.005&0.975&0.872&0.542&0.597&0.704&0.726&0.686&1.098&0.787 \\
EF-BLSTM & 1.103&1.105&0.975&0.906&1.053&1.018&1.069&0.999&0.882&0.580&0.607&0.742&0.762&0.705&1.085&0.762\\
EF-SBLSTM &  1.062&1.055&0.926&0.917&1.027&1.020&0.991&0.988&0.877&0.543&0.594&0.720&0.746&0.697&1.102&0.779\\
MV-LSTM	& 	1.029&1.098&0.971&0.944&1.082&0.976&1.012&0.998&0.877&0.523&0.625&0.703&0.792&0.687&1.163&0.770 \\
BC-LSTM		& 1.016&1.008&0.914&0.859&0.942&\textbf{0.905}&0.906&0.927&0.888&0.564&0.630&0.708&0.680&0.705&1.025&0.767	 \\
TFN  & 1.049&1.104&0.927&0.864&1.058&1.000&1.029&0.973&0.900&0.572&0.621&0.706&0.743&0.727&1.132&0.770\\
MFN			&
{0.952}&{0.993}&{0.882}&\textbf{0.835}&\textbf{0.903}&0.908&\textbf{0.886}&{0.913}&{0.821}&\textbf{0.521}&{0.566}&{0.679}&\textbf{0.665}&{0.654}&\textbf{0.981}&\textbf{0.727} \\  
\Xhline{0.5\arrayrulewidth}
{\pipelines } 	& 
\textbf{0.933}&\textbf{0.938}&\textbf{0.868}&{0.852}&{0.967}&{0.914}&{0.887}&\textbf{0.893}&\textbf{0.781}&{0.522}&\textbf{0.566}&\textbf{0.652}&{0.666}&\textbf{0.640}&{1.014}&{0.728} \\  
\Xhline{0.5\arrayrulewidth}
$\Delta_{SOTA}$	& \textcolor{gg}{$\downarrow $ \textbf{0.019}} & \textcolor{gg}{$\downarrow $ \textbf{0.055}} & \textcolor{gg}{$\downarrow $ \textbf{0.014}} & \textcolor{gray}{$\uparrow $ \textbf{0.017}} & \textcolor{gray}{$\downarrow $ \textbf{0.064}} & \textcolor{gray}{$\uparrow $ \textbf{0.009}} & \textcolor{gray}{$\downarrow $ \textbf{0.001}} & \textcolor{gg}{$\downarrow $ \textbf{0.020}} &\textcolor{gg}{$\downarrow $ \textbf{0.040}} & \textcolor{gray}{$\uparrow $ \textbf{0.001}} & \textcolor{gg}{$\downarrow $ \textbf{0.0}} & \textcolor{gg}{$\downarrow $ \textbf{0.027}} & \textcolor{gray}{$\uparrow $ \textbf{0.001}} & \textcolor{gg}{$\downarrow $ \textbf{0.014}} & \textcolor{gray}{$\uparrow $ \textbf{0.033}} & \textcolor{gray}{$\downarrow $ \textbf{0.001}}\\ 
\Xhline{0.5\arrayrulewidth}
%& 0.975&1.012&0.891&0.842&0.943&0.919&0.912&0.925&0.836&0.531&0.576&0.689&0.675&0.662&1.577&1.016&0.750 \\  \hline
\end{tabular}
\label{overall-3}
\end{table*}

\begin{table*}[!htbp]
\fontsize{7}{10}\selectfont
%\centering
\setlength\tabcolsep{1.3pt}
\begin{tabular}{l : *{16}{K{0.82cm}}}
\Xhline{0.5\arrayrulewidth}
Dataset & \multicolumn{16}{c}{\textbf{POM Speaker Personality Traits}} \\
Task & \multicolumn{1}{c}{Con} & \multicolumn{1}{c}{Pas} & \multicolumn{1}{c}{Voi} & \multicolumn{1}{c}{Dom} & \multicolumn{1}{c}{Cre} & \multicolumn{1}{c}{Viv} & \multicolumn{1}{c}{Exp} & \multicolumn{1}{c}{Ent} & \multicolumn{1}{c}{Res} & \multicolumn{1}{c}{Tru} & \multicolumn{1}{c}{Rel} & \multicolumn{1}{c}{Out} & \multicolumn{1}{c}{Tho} & \multicolumn{1}{c}{Ner} & \multicolumn{1}{c}{Per} & \multicolumn{1}{c}{Hum}\\
Metric  & \multicolumn{16}{c}{$r$} \\ 
\Xhline{0.5\arrayrulewidth}
Majority & -0.041&-0.029&-0.104&-0.031&-0.122&-0.044&-0.065&-0.105&0.006&-0.077&-0.024&-0.085&-0.130&0.097&-0.127&-0.069 \\
SVM	& 0.063&0.086&-0.004&0.141&0.113&0.076&0.134&0.141&0.166&0.168&0.104&0.066&0.134&0.068&0.064&0.147\\
DF	& 0.240&0.273&0.017&0.139&0.112&0.173&0.118&0.217&0.148&0.143&0.019&0.093&0.041&0.136&0.168&0.259 \\
EF-LSTM			& 0.200&0.302&0.031&0.079&0.170&0.244&0.265&0.240&0.142&0.062&0.083&0.152&0.260&0.105&0.217&0.227\\
EF-SLSTM & 0.221&0.327&0.042&0.151&0.177&0.239&0.268&0.248&0.204&0.069&0.092&0.215&0.252&0.159&0.218&0.196 \\
EF-BLSTM & 0.162&0.289&-0.034&0.135&0.191&0.279&0.274&0.231&0.184&0.154&0.093&0.147&0.245&0.166&0.243&0.272\\
EF-SBLSTM  & 0.174&0.310&0.021&0.088&0.170&0.224&0.261&0.241&0.155&0.163&0.097&0.120&0.215&0.121&0.216&0.171\\
MV-LSTM	& 0.358&0.416&0.131&0.146&0.280&0.347&0.323&0.326&0.295&0.237&0.119&0.238&0.284&0.258&0.239&0.317 \\
BC-LSTM		& 0.359&0.425&0.081&0.234&0.358&0.417&0.450&0.361&0.293&0.109&0.075&0.078&0.363&0.184&0.344&0.319\\
TFN &  0.089&0.201&0.030&0.020&0.124&0.204&0.171&0.223&-0.051&-0.064&0.114&0.060&0.048&-0.002&0.106&0.213 \\ 
MFN  &  {0.395}&{0.428}&{0.193}&{0.313}&\textbf{0.367}&\textbf{0.431}&{0.452}&{0.395}&{0.333}&\textbf{0.296}&{0.255}&{0.259}&\textbf{0.381}&{0.318}&\textbf{0.377}&\textbf{0.386}\\ 
\Xhline{0.5\arrayrulewidth} 
{\pipelines }  &  \textbf{0.441}&\textbf{0.502}&\textbf{0.247}&\textbf{0.342}&{0.355}&{0.414}&\textbf{0.470}&\textbf{0.396}&\textbf{0.446}&{0.247}&\textbf{0.291}&\textbf{0.345}&{0.376}&\textbf{0.379}&{0.327}&{0.346}\\ 
\Xhline{0.5\arrayrulewidth}
$\Delta_{SOTA}$	& \textcolor{gg}{$\uparrow $ \textbf{0.046}} & \textcolor{gg}{$\uparrow $ \textbf{0.074}} & \textcolor{gg}{$\uparrow $ \textbf{0.054}} & \textcolor{gg}{$\uparrow $ \textbf{0.029}} & \textcolor{gray}{$\downarrow $ \textbf{0.012}} & \textcolor{gray}{$\downarrow $ \textbf{0.017}} & \textcolor{gg}{$\downarrow $ \textbf{0.018}} & \textcolor{gg}{$\uparrow $ \textbf{0.001}} & \textcolor{gg}{$\uparrow $ \textbf{0.113}} &\textcolor{gray}{$\downarrow $ \textbf{0.049}} & \textcolor{gg}{$\uparrow $ \textbf{0.036}} & \textcolor{gg}{$\uparrow $ \textbf{0.086}} & \textcolor{gray}{$\downarrow $ \textbf{0.005}} & \textcolor{gg}{$\uparrow $ \textbf{0.061}}& \textcolor{gray}{$\downarrow $ \textbf{0.050}} & \textcolor{gray}{$\downarrow $ \textbf{0.040}} \\ \Xhline{0.5\arrayrulewidth}
\end{tabular}
\caption{Results for personality trait recognition on the POM dataset. The best results are highlighted in bold and $\Delta_{SOTA}$ shows the change in performance over previous state of the art. Improvements are highlighted in green. The \ours \ significantly outperforms the current state of the art across all evaluation metrics.}
\label{pom}
\end{table*}


==> tables/times.tex <==
\begin{table}[t!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{5.5pt}
\begin{tabular}{l c c}
\Xhline{3\arrayrulewidth}
Method       & GPU & CPU \\ 
\Xhline{0.1\arrayrulewidth}
% DF              &  0.368,0.323,0.356,0.442,0.366 & 0.506,0.393,0.498,0.772,0.369\\
% EF-LSTM			&  1.817,1.862,1.270,1.114,1.508 & 1.991,4.092,3.053,4.008,2.789\\
% MV-LSTM			&  0.344,0.599,0.511,0.480,0.515 & 1.981,1.543,1.372,1.820,1.654\\
% BC-LSTM         &  0.196,0.250,0.196,0.201,0.209 & 2.190,0.778,0.421,0.361,0.931\\ 
% TFN             &  2.906,3.022,2.967,3.017,3.273 & 17.304,12.716,10.209,10.669,12.736\\ 
% MARN      	&   & \\  
% MFN      		&   0.059296,0.059146,0.058834,0.059822, & \\  
% {\ours}      	&   & \\  
DF              &  686/0.371 = 1850 & 686/0.508 = 1350 \\
EF-LSTM			&  686/1.514 = 453 & 686/3.187 = 215 \\
MV-LSTM			&  686/0.490 = 1400 & 686/1.674 = 410 \\
BC-LSTM         &  686/0.210 = 3270 & 686/0.936 = 733 \\ 
TFN             &  686/3.037 = 226 & 686/12.727 = 53.9 \\ 
MARN      		&  686/\\ 
MFN      		&  \\ 
{\pipelines}      	&  \\  
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{FPS for model inference on the CMU-MOSI test set on a single Nvidia GeForce GTX 1080 Ti GPU and (whatever cpu configuration darius 2 is in) CPU, averaged over 5 trials.}
\label{times}
\end{table}
